Multi-Task Partially Supervised Learning for Super-Resolution and Semantic Segmentation on Earth Observation data

Super-resolution and semantic segmentation are known to benefit one another, especially in the Earth observation context. However, learning both tasks in a joint model often requires both task annotations, which is impractical and expensive. In this paper, we study the multi-task partially supervised learning paradigm for both tasks, where each example is assumed to have only a single-task annotation. To that end, we examine two multi-task architectural variations, the sequential and shared variants, and then propose a hybrid variant and a re-projection loss to benefit from the shared representation and enforce image quality of super-resolution when training with semantic segmentation. Experiments show favorable results compared to the SOTA sequential variant. Source code will be published at https://github.com/lhoangan/munera.

==> 0_definitions.tex <==

\newcommand{\pif}[1]{%
\begin{tikzpicture}
\draw (0,0) circle (1ex);
\end{tikzpicture}%
}
\newcommand{\pii}[1]{%
\begin{tikzpicture}
\draw[densely dotted] (0,0) circle (1ex);\draw (1ex,0) arc (0:#1:1ex) -- (0,0) -- cycle;
\end{tikzpicture}%
}
\newcommand{\pie}[1]{%
\begin{tikzpicture}
\draw[densely dotted] (0,0) circle (1ex);\draw[fill] (1ex,0) arc (0:#1:1ex) -- (0,0) -- cycle;
\end{tikzpicture}%
}
\newcommand{\pha}[1]{\phantom{\pie{#1}}}
\newcommand{\pik}[1]{%
\begin{tikzpicture}
 \draw (0,0) circle (1ex);\fill (1ex,0) arc (0:360:1ex) -- (0,0) -- cycle;
 \node[scale=.7] at (0,0) {\textcolor{white}{#1}};
\end{tikzpicture}%
}
\newcommand{\pic}{%
\begin{tikzpicture}
\draw[densely dotted] (0, 0) circle (1ex);
\draw[fill] (1ex ,0ex) -- (1ex,-1ex) arc(-90:90:1ex) -- (1ex, 0);
\end{tikzpicture}%
}
\newcommand{\hlefte}{%
\begin{tikzpicture}
\draw (0, 0) -- (0ex, 0ex) arc(90:270:1ex) -- (0, 0);
\end{tikzpicture}%
}
\newcommand{\hleft}{%
\begin{tikzpicture}
\draw[fill] (0, 0) -- (0ex, 0ex) arc(90:270:1ex) -- (0, 0);
\end{tikzpicture}%
}
\newcommand{\hleftk}{%
\begin{tikzpicture}
\draw[densely dotted] (0, -1ex) -- (-1ex, -1ex) arc(180:270:1ex) -- (0, -1ex) ;
\draw[fill]  (0, 0) arc(90:180:1ex) -- (0, -1ex) -- (0, 0);
\end{tikzpicture}%
}
\newcommand{\hright}{%
\begin{tikzpicture}
\draw[fill] (0, 0) -- (0ex, 0ex) arc(-90:90:1ex) -- (0, 0);
\end{tikzpicture}%
}
\newcommand{\hrightk}{%
\begin{tikzpicture}
\draw[densely dotted] (0, 0) arc(-90:90:1ex) -- (0, 0);
\draw[fill](0, 1ex) -- (1ex, 1ex) arc(0:90:1ex); 
\end{tikzpicture}%
}


==> Tables/Tab2_voc_half_quarter_eighth_full.tex <==
    \begin{tabular}{@{}lcrrrr@{}}
         \toprule
         Teacher                & \pha{360}  & \pie{180} 58.24 & \pie{ 90}    53.11 &  \pie{ 45} 46.42 \\ %
         \midrule
         \midrule
         Supervised             & \pie{180} &    51.08  &     47.16   &     39.82  \\ %
         \phantom{Hard}+MSE     &           &    53.40  &     48.88   &     41.83  \\ %
         \phantom{Hard}+PDF     &           &    54.18  &\bf  50.13   & \bf 42.81  \\ %
         \phantom{Hard}+DeFeat  &           &\bf 54.30  &     49.54   &     42.19  \\ %
         \midrule
         Self-trained           & \pif{360} &    55.64  &     51.82   &     46.59  \\ %
         \phantom{Soft}+MSE     &           &    55.53  &     51.41   &     46.21  \\ %
         \phantom{Soft}+PDF     &           &\bf 56.47  &\bf  51.93   & \bf 46.59  \\ %
         \phantom{Soft}+DeFeat  &           &    55.84  &     51.47   &     46.02  \\ %
         \bottomrule
    \end{tabular}


==> Tables/Tab3_voc_disjoint_half2.tex <==
    \begin{tabular}{@{}lcrrr@{}}
         \toprule
         Teacher               & \pha{360}  & \pie{180} 58.24 & \pie{ 90}    53.11 &  \pie{ 45} 46.42 \\ %
         \midrule
         \midrule
         Supervised            & \pie{180}  &    51.08  &     47.16 &     39.82  \\ %
         Self-trained          & \pii{-180} &     52.86 &     49.63 &     45.09 \\ %
         \phantom{Soft}+MSE    &            &     53.83 &     49.72 &     44.85 \\ %
         \phantom{Soft}+PDF    &            & \bf 54.26 & \bf 50.64 & \bf 45.63 \\ %
         \phantom{Soft}+DeFeat &            &     53.58 &     49.90 &     44.54 \\ %
         \bottomrule
    \end{tabular}





==> Tables/Tab4_voc_disjoint_ext.tex <==

\begin{tabular}{@{}lcccc@{}}
  \toprule
  Teacher              & \pie{180}      58.24 & \pie{ 90} 53.11      &  \pie{ 45}  46.42     &\pie{ 45}  46.42     \\ %
  \midrule                                                              
  \midrule                                                              
  Supervised           & \pie{180}      51.08 & \pie{180}      47.16 &  \pie{180}      39.82 &\pie{180}      39.82  \\ %
  Self-trained         & \pii{-180}     52.86 & \pii{-270}     51.23 &  \pii{-270}     46.28 &\pii{-305}     46.23 \\ %
  \phantom{Soft}+MSE   & \pha{-180}     53.83 & \pha{-270}     51.15 &  \pha{-270}     45.98 &\pha{-305}     46.24 \\ %
  \phantom{Soft}+PDF   & \pha{-180} \bf 54.26 & \pha{-270} \bf 51.34 &  \pha{-270} \bf 46.44 &\pha{-305} \bf 46.53 \\ %
  \phantom{Soft}+DeFeat& \pha{-180}     53.58 & \pha{-270}     51.02 &  \pha{-270}     45.94 &\pha{-305}     45.99 \\ %
  \bottomrule
\end{tabular}



==> Tables/Tab5_new_content.tex <==
\begin{tabular}{@{}lrrrr@{}}
     \toprule
     Teacher                   &&\hrightk\ 68.39 & \hright\ 71.12 & \hleftk\hright\ 72.40 \\ %
     \midrule
     \midrule
     Supervised       & \hleftk &          40.58 &          40.58 &     40.58 \\ %
     \phantom{Hard}+MSE        &&          42.54 &          42.55 &     42.91 \\ %
     \phantom{Hard}+DeFeat     &&     \bf  43.62 &      \bf 44.23 & \bf 44.73 \\ %
     \midrule
     Supervised       &\hleft   &          47.41 &          47.41 &     47.41 \\ %
     \phantom{Hard}+MSE        &&          48.53 &          49.04 &     49.36 \\ %
     \phantom{Hard}+DeFeat     &&     \bf  48.79 &      \bf 49.56 & \bf 49.79 \\ %
     \bottomrule
\end{tabular}


==> Tables/Tab6_new.tex <==
    \begin{tabular}{@{}llcccc@{}}
        \toprule
                                           && \multicolumn{2}{c}{Detection}   &\multicolumn{2}{c}{Segmentation} \\
        \midrule
        Teacher                            && \hleftk          &       49.99  &&      -           \\ %
        \midrule
        \midrule
        Supervised                         && \hleftk          &       40.45  & \hright& 65.04    \\ %
        $\quad$ pretrained on \hright      && \hleftk          &       41.00  &        &          \\ %
        \midrule
        Self-trained                       && \hlefte          &       43.08  &        &          \\ %
        $\quad$ pretrained on \hleftk      && \hlefte          &       44.15  &        &          \\ %
        \midrule
        Self-trained                       && \pif{360}        &       45.80  &        &          \\ %
        $\quad$ pretrained on \hleftk      && \pif{360}        &       46.50  &        &          \\ %
        \midrule
        Multitask                          &  \hleftk\hright  &&       45.63  &        &    65.53 \\ %
        $\quad$ pretrained on \hleftk      &  \hleftk\hright  &&       45.58  &        &    65.23 \\ %
        $\quad$ self-training DET          &  \hlefte\hright  &&       43.84  &        &\bf 70.53 \\ %
        $\qquad$ pretrained on \hleftk     &  \hlefte\hright  &&       45.47  &        &    69.83 \\ %
        $\qquad\quad$ + PDF \hleftk        &  \hlefte\hright  && \bf   47.77  &        &    67.37 \\ %
        \bottomrule
    \end{tabular}


==> Tables/Table3.tex <==


\begin{table}[t]
    \newcommand{\BlnRSR}{Real-SR~\cite{Ji20}}
    \newcommand{\BlnU}{USR-DA~\cite{Wang2021_USRDA}}
    \newcommand{\BlnSS}{sequential~\cite{Aakerberg2022}}
    \newcommand{\BlnRESR}{Real-ESR~\cite{Wang2021realesr}}
    \setlength{\tabcolsep}{1.5pt}
    \centering%
    \begin{tabular}{@{}llccccc@{}}
        \toprule
Input data      & Architecture& PMTL       &   SSIM    &   PSNR     &    mIOU    \\                                %
\midrule
\BlnRSR         & RRDBNet     &            &    60.107 &    20.141  &     - \\ %
\BlnU           & RRDBNet     &            &    63.091 &    24.397  &    - \\ %
\BlnRESR        & RRDBNet     &            &    75.632 &    25.318  &    -      \\ %
\BlnRESR        & hybrid      & \checkmark &    73.822 &    25.062  &    64.690 \\ %
\BlnRSR         & \BlnSS      & \checkmark &    68.941 &    21.309  &    62.663 \\ %
Bicubic         & hybrid      & \checkmark &    76.903 &\bf 26.338  &    64.512 \\ %
Bicubic  N2V    & hybrid      & \checkmark &\bf 81.272 &    24.250  &\bf 65.279 \\ %
        \bottomrule
    \end{tabular}
    \caption{Real-world super-resolution with $n\sim\mathcal{N}(0, 4)$. Our approach with the N2V teacher-student model outperforms the other baselines by large margins.}
    \vspace{-1em}
    \label{tab:Bld-G4-ISPRS}
\end{table}




==> _definitions.tex <==
\makeatletter
\RequirePackage{xspace}
\DeclareRobustCommand\onedot{\futurelet\@let@token\bmv@onedotaux}
\def\bmv@onedotaux{\ifx\@let@token.\else.\null\fi\xspace}
\makeatother


\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onnedot}
\def\etal{\emph{et al}\onedot}


\newcommand{\abbr}{CMG} %
\graphicspath{{./Images/}{./Figures/result/}{./Images/result/}}
\svgpath{{./Images/svg-inkscape/}}



\newcommand{\OLD}[1]{}

\newcommand{\TODO}[1]{{\color{blue}\textbf{TODO: }#1}}
\newcommand{\todo}[1]{\TODO{#1}}

\newcommand{\AL}[1]{{\color{teal}\textbf{ÂL: }#1}}
\newcommand{\al}[1]{\AL{#1}}

\newcommand{\update}[1]{{\color{black}#1}}
\newcommand{\new}[1]{{\color{black}#1}}

\newcommand{\cnes}[1]{{#1}}

\newcommand{\ua}{$\uparrow$}
\newcommand{\da}{$\downarrow$}
\renewcommand{\bf}{\bfseries}
\renewcommand{\paragraph}[1]{{\textbf{#1}$\quad$}}


\newcommand{\pie}[1]{%
\begin{tikzpicture}
 \draw (0,0) circle (1ex);\fill (1ex,0) arc (0:#1:1ex) -- (0,0) -- cycle;
\end{tikzpicture}%
}
\newcommand{\pha}[1]{\phantom{\pie{#1}}}
\newcommand{\pik}[1]{%
\begin{tikzpicture}
 \draw (0,0) circle (1ex);\fill (1ex,0) arc (0:360:1ex) -- (0,0) -- cycle;
 \node[scale=.7] at (0,0) {\textcolor{white}{#1}};
\end{tikzpicture}%
}
\newcommand{\hleft}{%
\begin{tikzpicture}
\draw[fill] (0, 0) -- (0ex, 0ex) arc(90:270:1ex) -- (0, 0);
\end{tikzpicture}%
}
\newcommand{\hleftk}{%
\begin{tikzpicture}
\draw[densely dotted] (0, 0) arc(90:270:1ex) -- (0, 0)  ; \draw[fill]  (0, 0) arc(90:180:1ex) -- (0, -1ex) -- (0, 0);
\end{tikzpicture}%
}
\newcommand{\hright}{%
\begin{tikzpicture}
\draw[fill] (0, 0) -- (0ex, 0ex) arc(-90:90:1ex) -- (0, 0);
\end{tikzpicture}%
}
\newcommand{\hrightk}{%
\begin{tikzpicture}
\draw[densely dotted] (0, 0) arc(-90:90:1ex) -- (0, 0);
\draw[fill](0, 1ex) -- (1ex, 1ex) arc(0:90:1ex); 
\end{tikzpicture}%
}


\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\csch}{csch}
\DeclareMathOperator{\asec}{asec}
\DeclareMathOperator{\acot}{acot}
\DeclareMathOperator{\acsc}{acsc}
\DeclareMathOperator{\acosh}{acosh}
\DeclareMathOperator{\asinh}{asinh}
\DeclareMathOperator{\atanh}{atanh}
\DeclareMathOperator{\asech}{asech}
\DeclareMathOperator{\acsch}{aCsch}
\DeclareMathOperator{\acoth}{aCoth} 

\newlength\myheight
\newlength\mydepth
\settototalheight\myheight{Xygp}
\settodepth\mydepth{Xygp}
\setlength\fboxsep{0pt}
\newcommand*\inlinegraphics[1]{%
  \settototalheight\myheight{Xygp}%
  \settodepth\mydepth{Xygp}%
  \raisebox{-\mydepth}{\includegraphics[height=\myheight]{#1}}%
}

\definecolor{attention}{HTML}{d4aa00}


==> colors.tex <==
\definecolor{CanvasBG}{HTML}{FAFAFA}

\definecolor{UnccGreen}{HTML}{00703C}
\definecolor{UnccGold}{HTML}{B3A369}
\definecolor{UnccLightGreen}{HTML}{C3D7A4}
\definecolor{UnccYellow}{HTML}{F0CB00}
\definecolor{UnccOrange}{HTML}{F3901D}
\definecolor{UnccLightYellow}{HTML}{FFF6DC}
\definecolor{UnccBlue}{HTML}{00728F}
\definecolor{UnccPink}{HTML}{DE3A6E}
\definecolor{White}{HTML}{FFFFFF}
\definecolor{LightGray}{HTML}{DDDDDD}

\definecolor{WarmGray}{HTML}{696158}
\definecolor{StoneGray}{HTML}{717C7D}
\definecolor{DarkGreen}{HTML}{2C5234}
\definecolor{LightGreen}{HTML}{509E2F}
\definecolor{BrightGold}{HTML}{F0CB00}

\definecolor{Royal}{HTML}{72246C}
\definecolor{Ocean}{HTML}{006BA6}
\definecolor{Flash}{HTML}{B52555}
\definecolor{Citrus}{HTML}{FFB81C}
\definecolor{Spring}{HTML}{CEDC00}

\definecolor{Garden}{HTML}{B7CE95}
\definecolor{Sand}{HTML}{F0E991}
\definecolor{Bloom}{HTML}{F1E6B2}
\definecolor{Clay}{HTML}{B7B09C}
\definecolor{Cloud}{HTML}{BAC5B9}


\definecolor{header}{HTML}{AFBBE1}%
\definecolor{maroon}{HTML}{800000}
\definecolor{greenDark}{HTML}{00712D}
\definecolor{frame_bg}{HTML}{FFF1DB}
\definecolor{blueDark}{HTML}{667BC6}%

\setbeamercolor{frametitle}{bg=maroon}
\setbeamercolor{progress bar}{bg=Garden, fg=maroon}
\setbeamercolor{alerted text}{fg=Flash}

\setbeamercolor{block title}{bg=LightBlue, fg=White}
\setbeamercolor{block title example}{bg=Ocean, fg=White}
\setbeamercolor{block title alerted}{bg=header, fg=White}
\setbeamercolor{block body}{bg=CanvasBG}

\metroset{titleformat=smallcaps, progressbar=foot}

\makeatletter
\setlength{\metropolis@progressinheadfoot@linewidth}{2pt}
\setlength{\metropolis@titleseparator@linewidth}{2pt}
\setlength{\metropolis@progressonsectionpage@linewidth}{2pt}

